SCALE: Synergized Collaboration of Asymmetric Language Translation Engines

In this paper, we introduce SCALE, a collaborative framework that connects compact Specialized Translation Models (STMs) and general-purpose Large Language Models (LLMs) as one unified translation engine. By introducing translation from STM into the triplet in-context demonstrations, SCALE unlocks refinement and pivoting ability of LLM, thus mitigating language bias of LLM and parallel data bias of STM, enhancing LLM speciality without sacrificing generality, and facilitating continual learning without expensive LLM fine-tuning. Our comprehensive experiments show that SCALE significantly outperforms both few-shot LLMs (GPT-4) and specialized models (NLLB) in challenging low-resource settings. Moreover, in Xhosa to English translation, SCALE experiences consistent improvement by a 4 BLEURT score without tuning LLM and surpasses few-shot GPT-4 by 2.5 COMET score and 3.8 BLEURT score when equipped with a compact model consisting of merely 600M parameters. SCALE could also effectively exploit the existing language bias of LLMs by using an English-centric STM as a pivot for translation between any language pairs, outperforming few-shot GPT-4 by an average of 6 COMET points across eight translation directions. Furthermore we provide an in-depth analysis of SCALE's robustness, translation characteristics, and latency costs, providing solid foundation for future studies exploring the potential synergy between LLMs and more specialized, task-specific models.

==> tables/refinement_highres.tex <==
\begin{table*}[thbp!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc|cccc}
\toprule
& \bf COMET-22 & \bf COMETKiwi & \textbf{BLEURT} & \bf spBLEU & \bf COMET-22 & \bf  COMETKiwi & \bf BLEURT  & \bf spBLEU\\ \hline
& \multicolumn{4}{c|}{eng\_Latn-deu\_Latn} & \multicolumn{4}{c}{deu\_Latn-eng\_Latn}  \\
NLLB   & 86.9 & 82.9 & 76.8 & 43.4 & 89.1 & 84.2 & 79.8 & 48.5  \\
M2M100 & 85.6 & 82.6 & 74.6 & 43.0 & 88.3 & 83.8 & 78.2 & 45.5  \\
\hdashline  
Microsoft &  &   &   &  &   &   \\
XGLM & 81.3 & 78.9 & 69.7 & 28.3 & 86.0 & 81.9 & 74.9 & 38.1    \\
GPT-3.5 &  &   &   &  &   &   \\
GPT-4 & 89.0 & 85.2 & 79.3 & 48.3 & 90.0 & 84.6 & 81.2 & 50.5  \\
ISCL  & 89.0 & 85.1 & 79.5 & 47.8 & 89.9 & 84.7 & 81.1 & 49.4 \\
\hline
& \multicolumn{4}{c|}{eng\_Latn-ces\_Latn} & \multicolumn{4}{c}{ces\_Latn-eng\_Latn}  \\
NLLB   & 90.1 & 84.8 & 80.3 & 38.6 & 88.4 & 85.5 & 78.6 & 44.1 \\
M2M100 & 88.2 & 83.2 & 77.3 & 38.8 & 87.3 & 84.6 & 76.6 & 41.0 \\
\hdashline  
Microsoft &  &   &   &  &   &   \\
XGLM   & 27.7 & 81.9 & 14.5 & 1.0 & 57.5 & 51.6 & 40.7 & 7.3   \\
GPT-3.5 &  &   &   &  &   &   \\
GPT-4 & 92.0 & 86.8 & 82.7 & 41.4 & 89.4 & 85.0 & 80.3 & 47.0  \\
ISCL  & 92.4 & 87.1 & 83.4 & 41.2 & 89.2 & 86.0 & 80.0 & 45.8 \\
% \hline
% & \multicolumn{4}{c|}{eng\_Latn-zho\_Hans} & \multicolumn{4}{c}{zho\_Hans-eng\_Latn}  \\
% NLLB  & 78.0 & 70.9 & 58.1 & 22.3 & 86.1 & 83.7 & 74.5 & 33.0 \\
% M2M100 & 83.4 & 80.8 & 67.3 & 27.8 & 85.0 & 82.9 & 72.3 & 27.7 \\
% \hdashline  
% Microsoft &  &   &   &  &   &   \\
% XGLM & 80.0 & 75.4 & 62.0 & 19.0 & 43.6 & 74.5 & 57.0 & 5.2 \\
% GPT-3.5 &  &   &   &  &   &   \\
% GPT-4 & 88.8 & 84.7 & 73.4 & 36.6 & 88.0 & 84.8 & 77.8 & 36.1  \\
% ISCL  & 89.1 & 84.7 & 73.6 & 37.2 & 87.8 & 84.9 & 77.4 & 35.1   \\
\hline
\end{tabular}
}
\label{table:refinement_highres}
\caption{Translation results of two high-resource languages.}
\end{table*}
